Improving Adaptive Seamless Designs through Bayesian optimization

We propose to use Bayesian optimization (BO) to improve the efficiency of the design selection process in clinical trials. BO is a method to optimize expensive black-box functions, by using a regression as a surrogate to guide the search. In clinical trials, planning test procedures and sample sizes is a crucial task. A common goal is to maximize the test power, given a set of treatments, corresponding effect sizes, and a total number of samples. From a wide range of possible designs we aim to select the best one in a short time to allow quick decisions. The standard approach to simulate the power for each single design can become too time-consuming. When the number of possible designs becomes very large, either large computational resources are required or an exhaustive exploration of all possible designs takes too long. Here, we propose to use BO to quickly find a clinical trial design with high power from a large number of candidate designs. We demonstrate the effectiveness of our approach by optimizing the power of adaptive seamless designs for different sets of treatment effect sizes. Comparing BO with an exhaustive evaluation of all candidate designs shows that BO finds competitive designs in a fraction of the time.

==> generated/tables/table_best.tex <==
\begin{table}

\caption{\label{tab:table_best}Best configurations per ncases and effects}
\centering
\fontsize{6}{8}\selectfont
\begin{tabular}[t]{lrlrrr}
\toprule
effect & n\_cases & select & stage\_ratio & epsilon & mean\_y\\
\midrule
 &  & epsilon rule & 0.042 & 0.000 & 0.401\\

 &  & 1 best & 0.083 &  & 0.405\\

 &  & epsilon rule & 0.083 & 0.000 & 0.407\\

 & \multirow{-4}{*}{\raggedleft\arraybackslash 500} & mbo &  &  & 0.422\\
\cmidrule{2-6}
 &  & epsilon rule & 0.083 & 0.167 & 0.729\\

 &  & 1 best & 0.083 &  & 0.731\\

 &  & epsilon rule & 0.083 & 0.000 & 0.735\\

 & \multirow{-4}{*}{\raggedleft\arraybackslash 1000} & mbo &  &  & 0.744\\
\cmidrule{2-6}
 &  & epsilon rule & 0.083 & 0.000 & 0.965\\

 &  & epsilon rule & 0.083 & 0.333 & 0.965\\

 &  & epsilon rule & 0.083 & 0.167 & 0.965\\

\multirow{-12}{*}{\raggedright\arraybackslash linear} & \multirow{-4}{*}{\raggedleft\arraybackslash 2000} & mbo &  &  & 0.970\\
\cmidrule{1-6}
 &  & 1 best & 0.125 &  & 0.417\\

 &  & epsilon rule & 0.083 & 0.167 & 0.421\\

 &  & epsilon rule & 0.083 & 0.000 & 0.424\\

 & \multirow{-4}{*}{\raggedleft\arraybackslash 500} & mbo &  &  & 0.435\\
\cmidrule{2-6}
 &  & epsilon rule & 0.167 & 0.500 & 0.719\\

 &  & epsilon rule & 0.125 & 0.500 & 0.723\\

 &  & epsilon rule & 0.125 & 0.333 & 0.728\\

 & \multirow{-4}{*}{\raggedleft\arraybackslash 1000} & mbo &  &  & 0.731\\
\cmidrule{2-6}
 &  & 2 best & 0.167 &  & 0.956\\

 &  & 2 best & 0.208 &  & 0.957\\

 &  & 2 best & 0.125 &  & 0.960\\

\multirow{-12}{*}{\raggedright\arraybackslash paper} & \multirow{-4}{*}{\raggedleft\arraybackslash 2000} & mbo &  &  & 0.965\\
\cmidrule{1-6}
 &  & 2 best & 0.208 &  & 0.915\\

 &  & 2 best & 0.292 &  & 0.917\\

 &  & 2 best & 0.250 &  & 0.919\\

 & \multirow{-4}{*}{\raggedleft\arraybackslash 500} & mbo &  &  & 0.929\\
\cmidrule{2-6}
 &  & 3 best & 0.250 &  & 0.998\\

 &  & 3 best & 0.208 &  & 0.998\\

 &  & 3 best & 0.167 &  & 0.998\\

 & \multirow{-4}{*}{\raggedleft\arraybackslash 1000} & mbo &  &  & 1.000\\
\cmidrule{2-6}
 &  & all & 0.042 &  & 1.000\\

 &  & 3 best & 0.042 &  & 1.000\\

 &  & all & 0.083 &  & 1.000\\

\multirow{-12}{*}{\raggedright\arraybackslash paper2} & \multirow{-4}{*}{\raggedleft\arraybackslash 2000} & mbo &  &  & 1.000\\
\cmidrule{1-6}
 &  & epsilon rule & 0.042 & 0.167 & 0.455\\

 &  & 1 best & 0.042 &  & 0.462\\

 &  & epsilon rule & 0.042 & 0.000 & 0.463\\

 & \multirow{-4}{*}{\raggedleft\arraybackslash 500} & mbo &  &  & 0.479\\
\cmidrule{2-6}
 &  & epsilon rule & 0.042 & 0.167 & 0.772\\

 &  & epsilon rule & 0.042 & 0.000 & 0.784\\

 &  & mbo &  &  & 0.787\\

 & \multirow{-4}{*}{\raggedleft\arraybackslash 1000} & 1 best & 0.042 &  & 0.794\\
\cmidrule{2-6}
 &  & epsilon rule & 0.042 & 0.167 & 0.972\\

 &  & 1 best & 0.042 &  & 0.977\\

 &  & mbo &  &  & 0.978\\

\multirow{-12}{*}{\raggedright\arraybackslash sigmoid} & \multirow{-4}{*}{\raggedleft\arraybackslash 2000} & epsilon rule & 0.042 & 0.000 & 0.979\\
\bottomrule
\end{tabular}
\end{table}

